Learning Better Visual Dialog Agents with Pretrained Visual-Linguistic Representation

GuessWhat?! is a two-player visual dialog guessing game where player A asks a sequence of yes/no questions (Questioner) and makes a final guess (Guesser) about a target object in an image, based on answers from player B (Oracle). Based on this dialog history between the Questioner and the Oracle, a Guesser makes a final guess of the target object. Previous baseline Oracle model encodes no visual information in the model, and it cannot fully understand complex questions about color, shape, relationships and so on. Most existing work for Guesser encode the dialog history as a whole and train the Guesser models from scratch on the GuessWhat?! dataset. This is problematic since language encoder tend to forget long-term history and the GuessWhat?! data is sparse in terms of learning visual grounding of objects. Previous work for Questioner introduces state tracking mechanism into the model, but it is learned as a soft intermediates without any prior vision-linguistic insights. To bridge these gaps, in this paper we propose Vilbert-based Oracle, Guesser and Questioner, which are all built on top of pretrained vision-linguistic model, Vilbert. We introduce two-way background/target fusion mechanism into Vilbert-Oracle to account for both intra and inter-object questions. We propose a unified framework for Vilbert-Guesser and Vilbert-Questioner, where state-estimator is introduced to best utilize Vilbert's power on single-turn referring expression comprehension. Experimental results show that our proposed models outperform state-of-the-art models significantly by 7%, 10%, 12% for Oracle, Guesser and End-to-End Questioner respectively.

==> post_analysis.tex <==
\section{Post Analysis}
As is shown in the ablation study (Table-\ref{tab:e2e_4_setting}), we observe that when either the Vilbert-Oracle model or Vilbert-Guesser model is introduced to the end-to-end game, the overall accuracy has shown no improvement over the baselines. Only when both proposed models are introduced in the game, the end-to-end accuracy has improved significantly (55.7\% over 47.7\%). 

\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
QGen & Oracle & Guesser & End-to-End Accuracy \\
\hline\hline
VDST & Baseline & Baseline & 47.7\% \\
VDST & Ours & Baseline & 47.8\% \\
VDST & Baseline & Ours & 47.5\% \\
VDST & Ours & Ours & 55.7\% \\
\hline
\end{tabular}
\end{center}
\caption{End-to-End Game Evaluation with Different Oracle and Guesser Models}
\label{tab:e2e_4_setting}
\end{table}

We conducted deep dive analysis to understand why introducing the single Vilbert-Oracle model or Vilbert-Guesser  did not bring benefit to the end-to-end evaluation.
\subsection{Introducing Only Vilbert-Guesser}

The Oracle model (either baseline Oracle or Our Vilbert-Oracle) output is not always correct in end-to-end evaluation. To simulate this effect in a controllable manner, we keep a fixed ground-truth dialog and randomly corrupt the ground-truth Oracle data with varying ratio (10\%-90\%). More specifically, we take the ground-truth dialogs with question and answer pairs, and randomly corrupt a portion of the answers with the following heuristics: (1) flip ground-truth answer to the opposite  (“Yes” → “No” and “No” → “Yes”); (2) replace “N/A” with random “Yes” or “No”. Then for each of the same corrupted dataset, we run both the baseline guesser and our Vilbert-Guesser to see to what extent the guesser modesl are sensitive to the corruption of Oracle answers. The results are depicted in Figure \ref{fig:guesser_on_corrupted_oracle}. 

From the results we can see that when the corruption ratio is low (10\%-40\%), our Vilbert-Guesser consistently outperforms the baseline Guesser. However, when the Oracle data is corrupted to a large ratio ($\geq$ 50\%), our Vilbert-Guesser degraded much faster than baseline model, suggesting that our model is more sensitive to the correctiveness of the Oracle model. This may explain why only introducing the Vilbert-Guesser didn’t improve end-to-end accuracy, since the baseline Oracle model might have relatively low accuracy, as is shown in independent evaluation section of Oracle models. 



\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1.0\linewidth]{method/figures/oracle_data_corruption.png}
\end{center}
   \caption{Performance of Two Guesser Models on Corrupted Oracle Data with Varying Corruption Ratios}
\label{fig:guesser_on_corrupted_oracle}
\end{figure}




\subsection{Introducing Only Vilbert-Oracle}
In end-to-end game, when a better Oracle model is introduced, the corresponding Guesser should also adapt to it and make a better guess. In our deep dive analysis we found that this holds true for our Vilbert-Guesser, but not the case for baseline Guesser. More specifically, we utilize the same QGen model (VDST), and generate dialogs with baseline Oracle and Vilbert Oracle respectively, and compute the confusion matrix using a baseline Guesser (Table-\ref{tab:confusion_matrix_baseline_guesser}) and using our Vilbert-Guesser (Table-\ref{tab:confusion_matrix_vilbert_guesser}). 







\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{latex/method/figures/venn_baseline_guesser.png}
  \caption{Using Baseline Guesser }
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{latex/method/figures/venn_vilbert_guesser.png}
  \caption{Using VilBert Guesser}
  \label{fig:sub2}
\end{subfigure}
\caption{Venn Chart Success Coverage Shifts between Baseline Guesser and VilBert Guesser}
\label{fig:test}
\end{figure}


From the confusion matrix (Table-\ref{tab:confusion_matrix_baseline_guesser}), we can observe that the baseline guesser make roughly similar amount of correct guesses and mistakes on dialogs generated by baseline Oracle and Vilbert-Oralce, with a small portion of non-overlaps (~1100 examples). But when we replace it with the Vilbert-Guesser (Table-\ref{tab:confusion_matrix_vilbert_guesser}), it makes less mistakes on the dialogs generated by Vilbert-Oracle, compared to those generated by baseline-Oracle (756 examples versus 2389 examples).

\begin{table}
\begin{center}
\begin{tabular}{|p{1.2 cm}|p{1.2 cm}|p{1.1cm}| p{1.1cm} | p{1cm} |}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}}&  \multicolumn{3}{c|}{Vilbert-Oracle}\\
\cline{3-5}
\multicolumn{2}{|c|}{} &  Correct &  Wrong & Total\\
\hline\hline
\multirow{3}{1.2cm}{Baseline Oracle} & Correct & 8391 & 1194 & 47.9\% \\
& Wrong & 1167 & 9243 & 52.1\% \\
& Total & 47.8\% & 52.2\% &  \\
\hline
\end{tabular}
\end{center}
\caption{Confusion Matrix of Baseline Guesser on End-to-End Dialogues Generated from Baseline Oracle and Vilbert-Oracle }
\label{tab:confusion_matrix_baseline_guesser}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\begin{center}
\begin{tabular}{|p{1.2 cm}|p{1.2 cm}|p{1.1cm}| p{1.1cm} | p{1cm} |}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}}&  \multicolumn{3}{c|}{Vilbert-Oracle}\\
\cline{3-5}
\multicolumn{2}{|c|}{} &  Correct &  Wrong & Total\\
\hline\hline
\multirow{3}{1.2cm}{Baseline Oracle} & Correct & 8749 & 756 & 47.5\% \\
& Wrong & 2389 & 8101 & 52.5\% \\
& Total & 55.7\% & 44.3\% &  \\
\hline
\end{tabular}
\end{center}
\caption{Confusion Matrix of Vilbert Guesser on End-to-End Dialogues Generated from Baseline Oracle and Vilbert-Oracle }
\label{tab:confusion_matrix_vilbert_guesser}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
\begin{tabular}{|p{1.2 cm}|p{1.2 cm}|p{1.1cm}| p{1.1cm} | p{1cm} |}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}}&  \multicolumn{3}{c|}{Vilbert-Guesser}\\
\cline{3-5}
\multicolumn{2}{|c|}{} &  Correct &  Wrong & Total\\
\hline\hline
\multirow{3}{1.2cm}{Baseline Guesser} & Correct & 7565 & 1993 & 47.8\% \\
& Wrong & 3573 & 6864 & 52.2\% \\
& Total & 55.7\% & 44.3\% &  \\
\hline
\end{tabular}
\end{center}
\caption{Confusion Matrix of End-to-End Dialogue Success Rate Generated from Baseline Guesser and Vilbert-Guesser Using Vilbert-Oracle }
\label{tab:confusion_matrix_vilbert_guesser}
\end{table}


Further, we manually examine the games that (1) baseline Guesser made mistakes on either Oracle settings; (2) Vilbert-Guesser makes mistakes on baseline Oracle settings but makes correct guess on Vilbert-Oracle settings. From these games, it shows that in many cases the Vilbert-Oracle generated the correct answer, but the baseline Guesser cannot make the correct guess while Vilbert-Guesser can (Table-4). 




\begin{table*}[t]
\begin{center}
\begin{tabular}{|p{7cm}|p{7cm}|}
\hline

\makecell[l]{
\raisebox{-\totalheight}{\includegraphics[width=0.4\textwidth]{latex/method/figures/7143.jpg}} \\
\textbf{Ground-truth object: 2} \\
\\
\textbf{Baseline Oracle + Baseline Guesser: 0} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|yes \\ \\
\textbf{Vilbert Oracle + Baseline Guesser:1} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|no \\ \\
\textbf{Baseline Oracle + Vilbert Guesser: 0} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|yes \\ \\
\textbf{Vilbert Oracle + Vilbert Guesser:2} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|no \\ \\
}  &

\makecell[l]{
\raisebox{-\totalheight}{\includegraphics[width=0.4\textwidth]{latex/method/figures/21146.jpg}} \\
\textbf{Ground-truth object: 2} \\
\\
\textbf{Baseline Oracle + Baseline Guesser: 1} \\
is it a person?|yes \\ 
is it a female?|yes \\ 
is she wearing a hat?|yes \\ \\
\textbf{Vilbert Oracle + Baseline Guesser:1} \\
is it a person?|yes \\ 
is it a female?|no \\ 
is it a man?|yes \\
is he wearing a hat?|yes \\ \\
\textbf{Baseline Oracle + Vilbert Guesser: 5} \\
is it a person?|yes \\ 
is it a female?|yes \\ 
is she wearing a hat?|yes \\ \\
\textbf{Vilbert Oracle + Vilbert Guesser:2} \\
is it a person?|yes \\ 
is it a female?|no \\ 
is it a man?|yes \\
is he wearing a hat?|yes \\ \\
}  \\


\hline
\end{tabular}
\end{center}
\caption{End-to-End Game Evaluation with Different Oracle and Guesser Models}
\label{tab:e2e_4_setting}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\iffalse
\begin{table*}[t]
\begin{center}
\begin{tabular}{|p{7cm}|p{7cm}|}
\hline

\makecell[l]{
\raisebox{-\totalheight}{\includegraphics[width=0.4\textwidth]{latex/method/figures/21146.jpg}} \\
\textbf{Ground-truth object: 2} \\
\\
\textbf{Baseline Oracle + Baseline Guesser: 1} \\
is it a person?|yes \\ 
is it a female?|yes \\ 
is she wearing a hat?|yes \\ \\
\textbf{Vilbert Oracle + Baseline Guesser:1} \\
is it a person?|yes \\ 
is it a female?|no \\ 
is it a man?|yes \\
is he wearing a hat?|yes \\ \\
\textbf{Baseline Oracle + Vilbert Guesser: 5} \\
is it a person?|yes \\ 
is it a female?|yes \\ 
is she wearing a hat?|yes \\ \\
\textbf{Vilbert Oracle + Vilbert Guesser:2} \\
is it a person?|yes \\ 
is it a female?|no \\ 
is it a man?|yes \\
is he wearing a hat?|yes \\ \\
}  &

\makecell[l]{
\raisebox{-\totalheight}{\includegraphics[width=0.4\textwidth]{latex/method/figures/24714.jpg}} \\
\textbf{Ground-truth object: 1} \\
\\
\textbf{Baseline Oracle + Baseline Guesser: 0} \\
is it a person?|yes \\ 
is it the person on the left?|no \\
is it the person on the right?|yes \\ \\
\textbf{Vilbert Oracle + Baseline Guesser:4} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|no \\
is it the person with the white shirt?|no \\
is it the person with the black shirt and black \\ pants?|yes \\ \\
\textbf{Baseline Oracle + Vilbert Guesser: 0} \\
is it a person?|yes \\ 
is it the person on the left?|no \\
is it the person on the right?|yes \\ \\
\textbf{Vilbert Oracle + Vilbert Guesser:1} \\
is it a person?|yes \\ 
is it the person on the left?|no \\ 
is it the person on the right?|no \\
is it the person with the white shirt?|no \\
is it the person with the black shirt and black \\ pants?|yes \\ \\
}  \\
\hline
\end{tabular}
\end{center}
\caption{End-to-End Game Evaluation with Different Oracle and Guesser Models}
\label{tab:e2e_4_setting}
\end{table*}
\fi

In summary, we observe this “Liebig’s barrel” effect among the Oracle agent and Guesser agent in the end-to-end games, namely, if only one of the two agents is “upgraded”, deemed in independent evaluation, there is no guarantee that the end-to-end performance can be improved, since the other “inferior” agent can still become the bottle-neck of the end-to-end performance. More specifically, when Vilbert-Guesser is introduced to work with the baseline Oracle, since baseline Oracle is more error-prone, and our Vilbert-Guesser is more sensitive to correctness of Oracle outputs, therefore it shows no improvement compared to using a baseline Guesser. Similarly, when Vilbert-Oracle is introduced to work with baseline guesser, we have shown that the baseline guesser often cannot make correct guesses even when Vilbert-Oracle is giving the correct answers. Only when both Vilbert-Oracle and Vilbert-Guesser models are introduced in the game, the bottle-neck has been mitigated, and thus producing better overall performance (55.7\%).

